MAD: Modality Agnostic Distance Measure for Image Registration

Multi-modal image registration is a crucial pre-processing step in many medical applications. However, it is a challenging task due to the complex intensity relationships between different imaging modalities, which can result in large discrepancy in image appearance. The success of multi-modal image registration, whether it is conventional or learning based, is predicated upon the choice of an appropriate distance (or similarity) measure. Particularly, deep learning registration algorithms lack in accuracy or even fail completely when attempting to register data from an "unseen" modality. In this work, we present Modality Agnostic Distance (MAD), a deep image distance}] measure that utilises random convolutions to learn the inherent geometry of the images while being robust to large appearance changes. Random convolutions are geometry-preserving modules which we use to simulate an infinite number of synthetic modalities alleviating the need for aligned paired data during training. We can therefore train MAD on a mono-modal dataset and successfully apply it to a multi-modal dataset. We demonstrate that not only can MAD affinely register multi-modal images successfully, but it has also a larger capture range than traditional measures such as Mutual Information and Normalised Gradient Fields.

==> mybibliography.tex <==
@article{Sotiras2013DeformableMI,
  title={Deformable Medical Image Registration: A Survey},
  author={A. Sotiras and C. Davatzikos and N. Paragios},
  journal={IEEE Transactions on Medical Imaging},
  year={2013},
  volume={32},
  pages={1153-1190}
}

@article{Xu2021RobustAG,
  title={Robust and Generalizable Visual Representation Learning via Random Convolutions},
  author={Z. Xu and D. Liu and J. Yang and M. Niethammer},
  journal={ICLR},
  year={2021},
}

@article{Doersch2015UnsupervisedVR,
  title={Unsupervised Visual Representation Learning by Context Prediction},
  author={C. Doersch and A. Gupta and A. Efros},
  journal={2015 IEEE International Conference on Computer Vision (ICCV)},
  year={2015},
  pages={1422-1430}
}

@inproceedings{Taleb2021MultimodalSL,
  title={Multimodal Self-Supervised Learning for Medical Image Analysis},
  author={A. Taleb and C. Lippert and T. Klein and M. Nabi},
  booktitle={Information Processing in Medical Imaging},
  year={2021}
}


@article{Zagoruyko2015LearningTC,
  title={Learning to compare image patches via convolutional neural networks},
  author={S. Zagoruyko and N. Komodakis},
  journal={2015 IEEE Conference on Computer Vision and Pattern Recognition (CVPR)},
  year={2015},
  pages={4353-4361}
}

@inproceedings{Simonovsky2016ADM,
  title={A Deep Metric for Multimodal Registration},
  author={M. Simonovsky and B. Guti{\'e}rrez-Becker and D. Mateus and N. Navab and N. Komodakis},
  booktitle={International Conference on Medical Image Computing and Computer-Assisted Intervention},
  year={2016}
}

@article{Cao2017DeformableIR,
  title={Deformable Image Registration Based on Similarity-Steered CNN Regression},
  author={X. Cao and J. Yang and J. Zhang and D. Nie and M. Kim and Q. Wang and D. Shen},
  journal={Medical image computing and computer-assisted intervention: International Conference on Medical Image Computing and Computer-Assisted Intervention},
  year={2017},
  volume={10433},
  pages={300-308}
}

@article{Haskins2018LearningDS,
  title={Learning deep similarity metric for 3D MR–TRUS image registration},
  author={G. Haskins and J. Kruecker and U. Kruger and S. Xu and P. Pinto and B. Wood and P. Yan},
  journal={International Journal of Computer Assisted Radiology and Surgery},
  year={2018},
  volume={14},
  pages={417-425}
}

@article{Cheng2015DeepSL,
  title={Deep similarity learning for multimodal medical images},
  author={X. Cheng and L. Zhang and Y. Zheng},
  journal={Computer Methods in Biomechanics and Biomedical Engineering: Imaging \& Visualization},
  year={2015}
}

@article{Haber2006IntensityGB,
  title={Intensity Gradient Based Registration and Fusion of Multi-modal Images},
  author={E. Haber and J. Modersitzki},
  journal={Medical image computing and computer-assisted intervention: International Conference on Medical Image Computing and Computer-Assisted Intervention},
  year={2006},
  volume={9 Pt 2},
  pages={726-33}
}

@article{Heinrich2012MINDMI,
  title={MIND: Modality independent neighbourhood descriptor for multi-modal deformable registration},
  author={M. Heinrich and M. Jenkinson and M. Bhushan and T. Matin and F. Gleeson and M. Brady and J. Schnabel},
  journal={Medical image analysis},
  year={2012},
  volume={16 7},
  pages={1423-35}
}

@article{Studholme1999AnOI,
  title={An overlap invariant entropy measure of 3D medical image alignment},
  author={C. Studholme and D. Hill and D. Hawkes},
  journal={Pattern Recognition},
  year={1999},
  volume={32},
  pages={71-86}
}


@article{Czolbe2020DeepSimSS,
  title={DeepSim: Semantic similarity metrics for learned image registration},
  author={Steffen Czolbe and Oswin Krause and Aasa Feragen},
  journal={ArXiv},
  year={2020},
  volume={abs/2011.05735}
}

@article{Lee2009LearningSM,
  title={Learning similarity measure for multi-modal 3D image registration},
  author={D. Lee and M. Hofmann and F. Steinke and Y. Altun and N. Cahill and B. Sch{\"o}lkopf},
  journal={2009 IEEE Conference on Computer Vision and Pattern Recognition},
  year={2009},
  pages={186-193}
}


@article{Wells1996MultimodalVR,
  title={Multi-modal volume registration by maximization of mutual information},
  author={W. Wells and P. Viola and H. Atsumi and S. Nakajima and R. Kikinis},
  journal={Medical image analysis},
  year={1996},
  volume={1 1},
  pages={35-51}
}

@article{Loeckx2010NonrigidIR,
  title={Nonrigid Image Registration Using Conditional Mutual Information},
  author={D. Loeckx and P. Slagmolen and F. Maes and D. Vandermeulen and P. Suetens},
  journal={IEEE Transactions on Medical Imaging},
  year={2010},
  volume={29},
  pages={19-29}
}

@article{Woo2015MultimodalRV,
  title={Multimodal Registration via Mutual Information Incorporating Geometric and Spatial Context},
  author={J. Woo and M. Stone and J. Prince},
  journal={IEEE Transactions on Image Processing},
  year={2015},
  volume={24},
  pages={757-769}
}

@article{Wachinger2012EntropyAL,
  title={Entropy and Laplacian images: Structural representations for multi-modal registration},
  author={C. Wachinger and N. Navab},
  journal={Medical image analysis},
  year={2012},
  volume={16 1},
  pages={1-17}
}

@article{Arar2020UnsupervisedMI,
  title={Unsupervised Multi-Modal Image Registration via Geometry Preserving Image-to-Image Translation},
  author={M. Arar and Y. Ginger and D. Danon and I. Leizerson and A. Bermano and D. Cohen-Or},
  journal={2020 IEEE/CVF Conference on Computer Vision and Pattern Recognition (CVPR)},
  year={2020},
  pages={13407-13416}
}

@article{Mok2022AffineMI,
  title={Affine Medical Image Registration with Coarse-to-Fine Vision Transformer},
  author={T. Mok and A. Chung},
  journal={2022 IEEE/CVF Conference on Computer Vision and Pattern Recognition (CVPR)},
  year={2022},
  pages={20803-20812}
}


@article{chen2019med3d,
    title={Med3D: Transfer Learning for 3D Medical Image Analysis},
    author={C. Sihong and M. Kai and Z. Yefeng},
    journal={arXiv preprint arXiv:1904.00625},
    year={2019}
}

@article{Sandkhler2018AirLabAI,
  title={AirLab: Autograd Image Registration Laboratory},
  author={R. Sandk{\"u}hler and C. Jud and S. Andermatt and P. Cattin},
  journal={ArXiv},
  year={2018},
}


@article{Kingma2015AdamAM,
  title={Adam: A Method for Stochastic Optimization},
  author={D. Kingma and J. Ba},
  journal={CoRR},
  year={2015},
}

@article{Shafto2014TheCC,
  title={The Cambridge Centre for Ageing and Neuroscience (Cam-CAN) study protocol: a cross-sectional, lifespan, multidisciplinary examination of healthy cognitive ageing},
  author={M. Shafto and L. Tyler and M. Dixon and Jason R. Taylor and J. Rowe and R. Cusack and A. Calder and W. Marslen-Wilson and J. Duncan and T. Dalgleish and R. Henson and C. Brayne and F. Matthews},
  journal={BMC Neurology},
  year={2014},
  volume={14}
}

@article{Taylor2017TheCC,
  title={The Cambridge Centre for Ageing and Neuroscience (Cam-CAN) data repository: Structural and functional MRI, MEG, and cognitive data from a cross-sectional adult lifespan sample},
  author={J. Taylor and N. Williams and R. Cusack and T. Auer and M. Shafto and M. Dixon and L. Tyler and Cam-CAN-Group and R. Henson},
  journal={Neuroimage},
  year={2017},
  volume={144},
  pages={262 - 269}
}

@article{Iglesias2011Robex,
    author = {J. Iglesias  and C. Liu  and P. Thompson and Z. Tu},
    year = {2011},
    month = {11},
    pages = {1617-1634},
    title = {Robust Brain Extraction Across Datasets and Comparison with Publicly Available Methods},
    volume = {30(9)},
    journal = {IEEE Transactions on Medical Imaging}
}

@article{Lowekamp2013TheDO,
  title={The Design of SimpleITK},
  author={B. Lowekamp and D. Chen and L. Ib{\'a}{\~n}ez and D. Blezek},
  journal={Frontiers in Neuroinformatics},
  year={2013},
  volume={7}
}

@article{Marcus2007OpenAS,
  title={Open Access Series of Imaging Studies (OASIS): Cross-sectional MRI Data in Young, Middle Aged, Nondemented, and Demented Older Adults},
  author={D. Marcus and T. Wang and J. Parker and J. Csernansky and J. Morris and R. Buckner},
  journal={Journal of Cognitive Neuroscience},
  year={2007},
  volume={19},
  pages={1498-1507}
}

@article{Hering2022Learn2RegCM,
  title={Learn2Reg: comprehensive multi-task medical image registration challenge, dataset and evaluation in the era of deep learning},
  author={A. Hering and L. Hansen and T. Mok and A. Chung and H. Siebert and S. Hager and A. Lange and S. Kuckertz and S. Heldmann and W. Shao and S. Vesal and M. Rusu and G. Sonn and T. Estienne and M. Vakalopoulou and L. Han and Y. Huang and M. Brudfors and Y. Balbastre and S. Joutard and M. Modat and G. Lifshitz and D. Raviv and J. Lv and Q. Li and V. Jaouen and D. Visvikis and C. Fourcade and M. Rubeaux and W. Pan and Z. Xu and B. Jian and F. De Benetti and M. Wodzinski and N. Gunnarsson and H. Qiu and Z. Li and C. Grossbrohmer and A. Hoopes and I. Reinertsen and Y. Xiao and B. Landman and Y. Huo and K. Murphy and B. van Ginneken and A. Dalca and M. Heinrich},
  journal={IEEE transactions on medical imaging},
  year={2022},
  volume={PP}
}

@article{Franceschi2018BilevelPF,
  title={Bilevel Programming for Hyperparameter Optimization and Meta-Learning},
  author={L. Franceschi and P. Frasconi and S. Salzo and R. Grazzi and M. Pontil},
  journal={ArXiv},
  year={2018},
}
@inproceedings{West1996ComparisonAE,
  title={Comparison and evaluation of retrospective intermodality image registration techniques.},
  author={J. West and J. Fitzpatrick and M. Wang and B. Dawant and C. Maurer and R. Kessler and R. Maciunas and C. Barillot and D. Lemoine and Andr{\'e} M. Collignon and F. Maes and P. Suetens and D. Vandermeulen and P. A. van den E. and P. Hemler and S. Napel and T. Sumanaweera and B. Harkness and D. Hill and C. Studholme and G. Malandain and X. Pennec and M. Noz and G. Maguire and M. Pollack and C. Pelizzari and R. Robb and D. Hanson and R. Woods},
  booktitle={Medical Imaging},
  year={1996}
}

@article{Muschelli2015ValidatedAB,
  title={Validated automatic brain extraction of head CT images},
  author={J. Muschelli and N. Ullman and W. Mould and P. Vespa and D. Hanley and C. Crainiceanu},
  journal={NeuroImage},
  year={2015},
  volume={114},
  pages={379-385}
}


@article{Vos2019ADL,
  title={A deep learning framework for unsupervised affine and deformable image registration},
  author={B. De Vos and F. Berendsen and M. Viergever and H. Sokooti and M. Staring and I. Isgum},
  journal={Medical Image Analysis},
  year={2019},
  volume={52},
  pages={128–143}
}

@book{Efron2016ComputerAS,
author = {E.Bradley and H. Trevor},
title = {Computer Age Statistical Inference: Algorithms, Evidence, and Data Science},
year = {2016},
publisher = {Cambridge University Press},
address = {USA},
}

@article{Cohen1969StatisticalPA,
  title={Statistical Power Analysis for the Behavioral Sciences},
  author={J. Cohen},
  journal={The SAGE Encyclopedia of Research Design},
  year={1969}
}


@article{Hering2021Learn2RegCM,
  title={Learn2Reg: Comprehensive Multi-Task Medical Image Registration Challenge, Dataset and Evaluation in the Era of Deep Learning},
  author={A. Hering and L. Hansen and T. Mok and A. Chung and H. Siebert and S. Hager and A. Lange and S. Kuckertz and S. Heldmann and W. Shao and S. Vesal and M. Rusu and G. Sonn and T. Estienne and M. Vakalopoulou and L. Han and Y. Huang and M. Brudfors and Y. Balbastre and S. Joutard and M. Modat and G. Lifshitz and Daniel R. and J. Lv and Q. Li and Vincent J. and D. Visvikis and C. Fourcade and M. Rubeaux and W. Pan and Z. Xu and B. Jian and F. De Benetti and M. Wodzinski and N. Gunnarsson and H. Qiu and Zeju Li and C. Grossbrohmer and A. Hoopes and I. Reinertsen and Y. Xiao and B. A. Landman and Y. Huo and K. Murphy and B. van Ginneken and A. Dalca and M. Heinrich},
  journal={IEEE Transactions on Medical Imaging},
  year={2021},
  volume={42},
  pages={697-712}
}
@inproceedings{he2016deep,
  title={Deep residual learning for image recognition},
  author={He, K. and Zhang, X. and Ren, S. and Sun, J.},
  booktitle={Proceedings of the IEEE conference on computer vision and pattern recognition},
  pages={770--778},
  year={2016}
}

@article{Pielawski2020CoMIRCM,
  title={CoMIR: Contrastive Multimodal Image Representation for Registration},
  author={Nicolas Pielawski and Elisabeth Wetzer and Johan Ofverstedt and Jiahao Lu and Carolina Wahlby and Joakim Lindblad and Natavsa Sladoje},
  journal={ArXiv},
  year={2020},
  volume={abs/2006.06325}
}

@inproceedings{Dey2022ContraRegCL,
  title={ContraReg: Contrastive Learning of Multi-modality Unsupervised Deformable Image Registration},
  author={Neel Dey and Jo Schlemper and Seyed Sadegh Mohseni Salehi and Bo Zhou and Guido Gerig and Michal Sofka},
  booktitle={International Conference on Medical Image Computing and Computer-Assisted Intervention},
  year={2022}
}

@inproceedings{Qin2019UnsupervisedDR,
  title={Unsupervised Deformable Registration for Multi-Modal Images via Disentangled Representations},
  author={Chen Qin and Bibo Shi and Rui Liao and Tommaso Mansi and Daniel Rueckert and Ali Kamen},
  booktitle={Information Processing in Medical Imaging},
  year={2019}
}

@article{Hoffmann2020SynthMorphLC,
  title={SynthMorph: Learning Contrast-Invariant Registration Without Acquired Images},
  author={Malte Hoffmann and Benjamin Billot and Douglas N. Greve and Juan Eugenio Iglesias and Bruce R. Fischl and Adrian V. Dalca},
  journal={IEEE transactions on medical imaging},
  year={2020},
  volume={41},
  pages={543 - 558}
}
